Observational constraints on the stellar recycled gas in active galactic nuclei feeding

Near-infrared long-slit spectroscopy has been used to study the stellar population (SP) of the low luminosity active galactic nuclei (AGN) and matched analogues (LLAMA) sample. To perform the SP fits we have employed the X-shooter simple stellar population models together with the \st\ code. Our main conclusions are: The star formation history of the AGNs is very complex, presenting many episodes of star formation during their lifetimes. In general, AGN hosts have higher fractions of intermediate-age SP (light-weighted mean ages, $<t>_L\lesssim$ 4.5 Gyr) when compared with their analogues ($<t>_L\lesssim$ 8.0 Gyr). AGN are more affected by reddening and require significant fractions of featureless continuum and hot dust components. The ratio between the AGN radiated energy and the gravitational potential energy of the molecular gas ($E_{Rad}$/$E_{PG}$) for the AGN is compared with the \maL\ and a possible anti-correlation is observed. This suggests that the AGN is affecting the star formation in these galaxies, in the sense that more energetic AGN (log$(E_{Rad}$/$E_{PG}) \gtrsim 3$) tend to host nuclear younger SP ($ <t>_L \lesssim$4Gyr). We found that the recent ($t<$2~Gyr) returned (recycled) stellar mass is higher in AGN than in the controls. We also provide evidence that the mass loss of stars would be enough to feed the AGN, thus providing observational constraints for models that predict that AGN feeding is partially due to the recycled gas from dying stars.

==> sections/online.tex <==
\newpage

\appendix
\section{Final reduced spectra}

We present the remaining final reduced data from Fig.~\ref{apen_block1} to Fig.~\ref{apen_block10}. 

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO021-G004.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO137-G034.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/MCG-05-14-012.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/MCG-05-23-016.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the AGNs in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy, we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block1}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/MCG-06-30-015.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1365.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2110.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2992.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the AGNs in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy, we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block2}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3081.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3783.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4235.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4388.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the AGNs in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block3}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4593.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5128.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5506.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5728.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the AGNs in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H$, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block4}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC6814.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC7172.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC7213.pdf}
  \end{minipage}\hfill
  % Add a blank minipage for spacing if there is an odd number of images
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=\textwidth]{figures/NGC7582.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the AGNs in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block5}
\end{figure*}


%%%%%%%%%% CONTROLS %%%%%%%%%%%%%%%%%%%%%


\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO093-G003.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO208-G021.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/IC4653.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC0718.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the control galaxies in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block6}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1079.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1315.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1947.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2775.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the control galaxies in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block7}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3175.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3351.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3717.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3749.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the control galaxies in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block8}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4224.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4254.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4260.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5037.pdf}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the control galaxies in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block9}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5845.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5921.pdf}
  \end{minipage}\hfill
  % Add blank minipages for spacing if there is an odd number of images
  \begin{minipage}[b]{0.5\linewidth}
\includegraphics[width=\textwidth]{figures/NGC7727.pdf}
     \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
  \end{minipage}\hfill
  \caption{Final reduced spectra for the control galaxies in our sample in the Earth's velocity frame and corrected for galactic reddening. The sources are labeled. For each galaxy we show from top to bottom the $J$, $H $, and $K$ bands, respectively. The flux is in units of  $\rm 10^{-15}~ erg ~ cm^{-2} ~ s^{-1}$. The shaded grey area represents the uncertainties and the brown area shows the poor transmission region between different bands.}
  \label{apen_block10}
\end{figure*}



==> sections/online_SPS.tex <==
\newpage
\section{Individual Stellar Population fits}

We present the remaining individual stellar population fits from Fig.~\ref{app_sp1} to Fig.~\ref{app_sp10}.



\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO021-G004_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO137-G034_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2992_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/MCG-05-23-016_sint.pdf}
  \end{minipage}\hfill
  \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp1}
  \end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/MCG-06-30-015_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1365_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2110_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/MCG-05-14-012_sint.pdf}
  \end{minipage}\hfill
    \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp2}  
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3081_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3783_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2992_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4388_sint.pdf}
  \end{minipage}\hfill
    \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp3}  
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4593_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5128_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5506_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5728_sint.pdf}
  \end{minipage}\hfill
   \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
  \label{app_sp4}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC6814_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC7172_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC7213_sint.pdf}
  \end{minipage}\hfill
  % Add a blank minipage for spacing if there is an odd number of images
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=\textwidth]{figures/NGC7582_sint.pdf}
  \end{minipage}\hfill
   \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
  
 \label{app_sp5}
\end{figure*}


%%%%%%%%%% CONTROLS %%%%%%%%%%%%%%%%%%%%%


\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO093-G003_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/ESO208-G021_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/IC4653_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC0718_sint.pdf}
  \end{minipage}\hfill
  \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
  
\label{app_sp6}
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1079_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1315_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC1947_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC2775_sint.pdf}
  \end{minipage}\hfill
  \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp7}  
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3175_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3351_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3717_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC3749_sint.pdf}
  \end{minipage}\hfill
  \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp8}  
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4224_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4254_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC4260_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5037_sint.pdf}
  \end{minipage}\hfill
  \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp9}  
\end{figure*}

\begin{figure*}
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5845_sint.pdf}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/NGC5921_sint.pdf}
  \end{minipage}\hfill
  % Add blank minipages for spacing if there is an odd number of images
  \begin{minipage}[b]{0.5\linewidth}
\includegraphics[width=\textwidth]{figures/NGC7727_sint.pdf}
     \end{minipage}\hfill
  \begin{minipage}[b]{0.5\linewidth}
  \end{minipage}\hfill
   \caption{Spectral fitting results for the labelled galaxies for the original spectrum (see main text for details). For {\bf each galaxy}, on 
{\it top panel}: observed (black) and synthetic (red) spectra, light-weighted mean age, and metallicity.
{\it middle panel}: emission-line free spectrum (observed$-$synthetic spectrum) and a horizontal line showing the zero point for the continuum. 
{\it bottom panel}: from left to right, SFH summed over all metalicities in light ($x$) and in mass ($\mu$) fractions; SFH considering different metallicities; binned population vectors; AGN feature-less continuum and hot-dust contributions are on the two last panels. }
\label{app_sp10}  
  
\end{figure*}



==> sections/tab_SP_FULL.tex <==
\begin{table*}
\centering
\renewcommand{\tabcolsep}{.50mm}
\caption{Properties obtained fitting the full spectral range.}
\label{tab:spfitsFull}
\begin{tabular}{lccccccccccccccccc}
\noalign{\smallskip}
\hline
Source   &   xy   &  xiy   &  xio   &  xo   &  $\mu$y   &  $\mu$iy   &  $\mu$io   &  $\mu$o   &  FC    &  HD   & $<t>_L$   &  $<t>_M$  & $<Z>_L$        &  $<Z>_L$   &  $\chi^2_{red}$   &  Adev   &  Av      \\
         & (\%)   & (\%)   & (\%)   & (\%)  & (\%)      & (\%)       & (\%)       & (\%)      & (\%)    & (\%) & (Gyr)      & (Gyr)    & ($Z_{\odot}$)  & 	($Z_{\odot}$) &    	         & (\%)    &  (mag) \\  
\noalign{\smallskip}
\multicolumn{18}{c}{Sample} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
NGC2110 & 0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   58$\pm$0   &   0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   42$\pm$0   &   0$\pm$0   &   10.30$\pm$0.52   &   10.60$\pm$0.41   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   8$\pm$11   &   4.8$\pm$4.1   &   0.60$\pm$0.01   \\
NGC2992 & 0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   85$\pm$0   &   0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   13$\pm$0   &   2$\pm$0   &   12.30$\pm$0.00   &   12.30$\pm$0.00   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   4$\pm$1   &   3.2$\pm$0.5   &   1.53$\pm$0.01   \\
MCG-05-23-016 & 5$\pm$2   &   0$\pm$0   &   0$\pm$0   &   77$\pm$11   &   0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   17$\pm$13   &   1$\pm$0   &   8.56$\pm$1.23   &   11.60$\pm$0.32   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   2$\pm$1   &   6.9$\pm$0.8   &   0.89$\pm$0.04   \\
NGC3081 & 0$\pm$0   &   0$\pm$0   &   1$\pm$0   &   69$\pm$0   &   0$\pm$0   &   0$\pm$0   &   1$\pm$0   &   99$\pm$0   &   30$\pm$0   &   0$\pm$0   &   8.96$\pm$0.20   &   9.25$\pm$0.20   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   9$\pm$2   &   3.0$\pm$0.0   &   0.60$\pm$0.00   \\
ESO021-G004 & 0$\pm$0   &   8$\pm$5   &   15$\pm$9   &   78$\pm$4   &   0$\pm$0   &   4$\pm$3   &   13$\pm$7   &   83$\pm$5   &   0$\pm$0   &   0$\pm$0   &   2.30$\pm$0.13   &   2.54$\pm$0.11   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   39$\pm$8   &   12.6$\pm$4.8   &   1.50$\pm$0.05   \\
NGC5728 & 0$\pm$0   &   33$\pm$1   &   0$\pm$0   &   64$\pm$1   &   0$\pm$0   &   7$\pm$1   &   0$\pm$0   &   93$\pm$1   &   0$\pm$0   &   3$\pm$0   &   2.78$\pm$0.11   &   8.15$\pm$0.17   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   2$\pm$1   &   7.9$\pm$2.8   &   1.07$\pm$0.01   \\
ESO137-G034 & 0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   0$\pm$0   &   0$\pm$0   &   9.78$\pm$1.03   &   9.98$\pm$1.05   &   0.00$\pm$0.00   &   0.00$\pm$0.00   &   46$\pm$11   &   10.2$\pm$1.5   &   0.45$\pm$0.03   \\
NGC7172 & 0$\pm$0   &   5$\pm$1   &   24$\pm$1   &   46$\pm$1   &   0$\pm$0   &   2$\pm$0   &   16$\pm$1   &   82$\pm$1   &   0$\pm$0   &   26$\pm$0   &   3.32$\pm$0.12   &   5.47$\pm$0.28   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   6$\pm$1   &   3.2$\pm$0.7   &   1.99$\pm$0.02   \\
NGC7582 & 0$\pm$0   &   41$\pm$1   &   4$\pm$1   &   0$\pm$0   &   0$\pm$0   &   86$\pm$3   &   14$\pm$3   &   0$\pm$0   &   43$\pm$0   &   12$\pm$0   &   0.33$\pm$0.01   &   0.40$\pm$0.01   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   6$\pm$1   &   2.6$\pm$0.0   &   1.61$\pm$0.01   \\
\hline
\noalign{\smallskip}
\multicolumn{18}{c}{Control Sample} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
ESO093-G003 & 0$\pm$0   &   0$\pm$0   &   16$\pm$2   &   84$\pm$2   &   0$\pm$0   &   0$\pm$0   &   14$\pm$2   &   86$\pm$2   &   0$\pm$0   &   0$\pm$0   &   2.42$\pm$0.05   &   2.46$\pm$0.07   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   7$\pm$1   &   5.2$\pm$0.3   &   1.12$\pm$0.01   \\
ESO208-G021 & 0$\pm$0   &   0$\pm$1   &   17$\pm$3   &   82$\pm$2   &   0$\pm$0   &   0$\pm$0   &   5$\pm$1   &   95$\pm$1   &   0$\pm$0   &   0$\pm$0   &   8.56$\pm$0.37   &   11.20$\pm$0.20   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   1$\pm$1   &   6.9$\pm$0.5   &   0.79$\pm$0.01   \\
IC4653 & 44$\pm$4   &   20$\pm$5   &   21$\pm$5   &   15$\pm$2   &   19$\pm$3   &   15$\pm$4   &   36$\pm$9   &   30$\pm$5   &   0$\pm$0   &   0$\pm$0   &   0.24$\pm$0.02   &   0.65$\pm$0.07   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   5$\pm$2   &   7.4$\pm$0.2   &   0.19$\pm$0.04   \\
NGC0718 & 0$\pm$0   &   0$\pm$0   &   48$\pm$0   &   52$\pm$0   &   0$\pm$0   &   0$\pm$0   &   27$\pm$0   &   73$\pm$0   &   0$\pm$0   &   0$\pm$0   &   4.19$\pm$0.05   &   6.42$\pm$0.15   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   8$\pm$2   &   2.9$\pm$0.2   &   0.73$\pm$0.00   \\
NGC1079 & 0$\pm$0   &   1$\pm$2   &   18$\pm$4   &   77$\pm$2   &   0$\pm$0   &   0$\pm$1   &   7$\pm$2   &   92$\pm$1   &   0$\pm$0   &   4$\pm$0   &   4.85$\pm$0.52   &   6.76$\pm$0.89   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   1$\pm$0   &   42.1$\pm$10.8   &   0.66$\pm$0.02   \\
NGC1315 & 0$\pm$0   &   0$\pm$0   &   13$\pm$1   &   87$\pm$1   &   0$\pm$0   &   0$\pm$0   &   5$\pm$0   &   95$\pm$0   &   0$\pm$0   &   0$\pm$0   &   9.32$\pm$0.12   &   11.20$\pm$0.08   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   1$\pm$0   &   6.4$\pm$0.3   &   0.43$\pm$0.01   \\
NGC1947 & 0$\pm$0   &   0$\pm$0   &   12$\pm$2   &   88$\pm$2   &   0$\pm$0   &   0$\pm$0   &   10$\pm$2   &   90$\pm$2   &   0$\pm$0   &   0$\pm$0   &   2.91$\pm$0.04   &   2.95$\pm$0.04   &   0.01$\pm$0.00   &   0.01$\pm$0.00   &   1$\pm$1   &   10.4$\pm$6.3   &   2.06$\pm$0.00   \\
NGC2775 & 0$\pm$0   &   0$\pm$0   &   2$\pm$1   &   98$\pm$1   &   0$\pm$0   &   0$\pm$0   &   1$\pm$0   &   99$\pm$0   &   0$\pm$0   &   0$\pm$0   &   9.50$\pm$0.10   &   9.83$\pm$0.15   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   4$\pm$1   &   2.8$\pm$0.0   &   0.33$\pm$0.00   \\
NGC3175 & 0$\pm$0   &   61$\pm$0   &   0$\pm$0   &   37$\pm$0   &   0$\pm$0   &   25$\pm$1   &   0$\pm$0   &   75$\pm$1   &   0$\pm$0   &   2$\pm$0   &   0.94$\pm$0.02   &   3.77$\pm$0.23   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   3$\pm$1   &   3.9$\pm$0.0   &   1.92$\pm$0.00   \\
NGC3351 & 0$\pm$0   &   6$\pm$1   &   24$\pm$1   &   69$\pm$1   &   0$\pm$0   &   2$\pm$0   &   12$\pm$1   &   86$\pm$0   &   0$\pm$0   &   0$\pm$0   &   3.39$\pm$0.08   &   5.25$\pm$0.21   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   6$\pm$1   &   3.0$\pm$0.5   &   1.01$\pm$0.00   \\
NGC3717 & 0$\pm$1   &   30$\pm$2   &   0$\pm$0   &   67$\pm$2   &   0$\pm$0   &   6$\pm$1   &   0$\pm$0   &   94$\pm$1   &   0$\pm$0   &   3$\pm$0   &   2.66$\pm$0.18   &   7.67$\pm$0.27   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   2$\pm$0   &   2.8$\pm$0.2   &   2.32$\pm$0.03   \\
NGC3749 & 0$\pm$0   &   14$\pm$3   &   20$\pm$3   &   66$\pm$3   &   0$\pm$0   &   4$\pm$1   &   7$\pm$1   &   89$\pm$1   &   1$\pm$0   &   0$\pm$0   &   4.68$\pm$0.37   &   8.76$\pm$0.29   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   2$\pm$0   &   2.3$\pm$0.2   &   2.42$\pm$0.03   \\
NGC4224 & 0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   0$\pm$0   &   0$\pm$0   &   0$\pm$0   &   100$\pm$0   &   0$\pm$0   &   0$\pm$0   &   11.10$\pm$0.13   &   11.80$\pm$0.06   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   2$\pm$2   &   5.2$\pm$0.1   &   0.45$\pm$0.01   \\
NGC4254 & 0$\pm$0   &   0$\pm$0   &   52$\pm$1   &   48$\pm$1   &   0$\pm$0   &   0$\pm$0   &   24$\pm$1   &   76$\pm$1   &   0$\pm$0   &   0$\pm$0   &   3.18$\pm$0.06   &   6.21$\pm$0.11   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   7$\pm$1   &   3.8$\pm$0.4   &   0.72$\pm$0.01   \\
NGC5037 & 0$\pm$0   &   2$\pm$1   &   27$\pm$1   &   71$\pm$1   &   0$\pm$0   &   0$\pm$0   &   11$\pm$1   &   89$\pm$1   &   0$\pm$0   &   0$\pm$0   &   5.46$\pm$0.11   &   7.92$\pm$0.19   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   1$\pm$0   &   3.7$\pm$0.4   &   1.19$\pm$0.01   \\
NGC5845 & 0$\pm$0   &   0$\pm$0   &   13$\pm$1   &   87$\pm$1   &   0$\pm$0   &   0$\pm$0   &   4$\pm$0   &   96$\pm$0   &   0$\pm$0   &   0$\pm$0   &   7.18$\pm$0.19   &   9.08$\pm$0.24   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   7$\pm$1   &   2.6$\pm$0.0   &   0.42$\pm$0.00   \\
NGC5921 & 2$\pm$1   &   5$\pm$1   &   38$\pm$2   &   54$\pm$1   &   0$\pm$0   &   2$\pm$0   &   18$\pm$1   &   80$\pm$1   &   0$\pm$0   &   0$\pm$0   &   3.16$\pm$0.06   &   6.30$\pm$0.20   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   5$\pm$1   &   2.1$\pm$0.0   &   0.48$\pm$0.01   \\
NGC7727 & 0$\pm$0   &   0$\pm$0   &   12$\pm$0   &   88$\pm$0   &   0$\pm$0   &   0$\pm$0   &   4$\pm$0   &   96$\pm$0   &   0$\pm$0   &   0$\pm$0   &   7.77$\pm$0.11   &   9.56$\pm$0.19   &   0.02$\pm$0.00   &   0.02$\pm$0.00   &   7$\pm$1   &   2.8$\pm$0.4   &   0.49$\pm$0.00   \\
\hline
\end{tabular}
	\begin{list}{Table Notes:}
	\item notes
	\end{list}




\end{table*}


